Improving DRAM Performance by Parallelizing Refreshes with Accesses

Modern DRAM cells are periodically refreshed to prevent data loss due to leakage. Commodity DDR DRAM refreshes cells at the rank level. This degrades performance significantly because it prevents an entire rank from serving memory requests while being refreshed. DRAM designed for mobile platforms, LPDDR DRAM, supports an enhanced mode, called per-bank refresh, that refreshes cells at the bank level. This enables a bank to be accessed while another in the same rank is being refreshed, alleviating part of the negative performance impact of refreshes. However, there are two shortcomings of per-bank refresh. First, the per-bank refresh scheduling scheme does not exploit the full potential of overlapping refreshes with accesses across banks because it restricts the banks to be refreshed in a sequential round-robin order. Second, accesses to a bank that is being refreshed have to wait. To mitigate the negative performance impact of DRAM refresh, we propose two complementary mechanisms, DARP (Dynamic Access Refresh Parallelization) and SARP (Subarray Access Refresh Parallelization). The goal is to address the drawbacks of per-bank refresh by building more efficient techniques to parallelize refreshes and accesses within DRAM. First, instead of issuing per-bank refreshes in a round-robin order, DARP issues per-bank refreshes to idle banks in an out-of-order manner. Furthermore, DARP schedules refreshes during intervals when a batch of writes are draining to DRAM. Second, SARP exploits the existence of mostly-independent subarrays within a bank. With minor modifications to DRAM organization, it allows a bank to serve memory accesses to an idle subarray while another subarray is being refreshed. Extensive evaluations show that our mechanisms improve system performance and energy efficiency compared to state-of-the-art refresh policies and the benefit increases as DRAM density increases.

==> plots/dram-organization.tex <==
\begin{figure}[t]
%\begin{minipage}{\linewidth}
\footnotesize
\begin{center}
%\includegraphics[width=1.0\linewidth]{plots/dram-organization}
\includegraphics[scale=0.8]{plots/dram-organization}
\end{center}
\caption{DRAM memory system organization.}
\label{fig:dram-organization}
%\end{minipage}
\end{figure}


==> plots/main-scurves.tex <==
\begin{figure*}[t]
        \centering
        \subfloat[8Gb.]{
            \begin{minipage}{0.325\textwidth}
            \begin{center}
            \includegraphics[width=\textwidth]{plots/scurve_8gb}
            \vspace{-0.1in}
            \label{fig:8Gb-scurve}
            \end{center}
            \end{minipage}
        }
        %
        \subfloat[16Gb.]{
            \begin{minipage}{0.325\textwidth}
            \begin{center}
            \includegraphics[width=\textwidth]{plots/scurve_16gb}
            \vspace{-0.1in}
            \label{fig:16Gb-scurve}
            \end{center}
            \end{minipage}
        }
        %
        \subfloat[32Gb.]{
            \begin{minipage}{0.325\textwidth}
            \begin{center}
            \includegraphics[width=\textwidth]{plots/scurve_32gb}
            \vspace{-0.1in}
            \label{fig:32Gb-scurve}
            \end{center}
            \end{minipage}
        }
        %

        \caption{Multi-core system performance improvement over baseline
        all-bank refresh using various DRAM density.}\label{fig:scurves}
\end{figure*}

% Vertically stacked
%\begin{figure}[t]
%    \begin{tabular}{c}
%        \subfloat[8Gb.]{
%            \begin{minipage}{\linewidth}
%            \begin{center}
%            \includegraphics[scale=0.8]{plots/scurve_8gb}
%            \label{fig:8Gb-scurve}
%            \end{center}
%            \end{minipage}
%        } \\
%
%        \subfloat[16Gb.]{
%            \begin{minipage}{\linewidth}
%            \begin{center}
%            \includegraphics[scale=0.8]{plots/scurve_16gb}
%            \label{fig:16Gb-scurve}
%            \end{center}
%            \end{minipage}
%        } \\
%
%        \subfloat[32Gb.]{
%            \begin{minipage}{\linewidth}
%            \begin{center}
%            \includegraphics[scale=0.8]{plots/scurve_32gb}
%            \label{fig:32Gb-scurve}
%            \end{center}
%            \end{minipage}
%        } \\
%
%    \end{tabular}
%
%    \caption{Multi-core system performance improvement over baseline
%    all-bank refresh using various DRAM density.}
%    \label{fig:scurves}
%\end{figure}


==> plots/memory-organization.tex <==
%\begin{figure}[h]
%  \centering
%
%  \subfigure[DRAM Memory System Organization.]{
%  \label{fig:dram-organization}
%  \includegraphics[width=\linewidth]{figures/dram-organization}
%  }
%  \subfigure[]{
%  \label{fig:bank-subarray}
%  \includegraphics[width=0.85\linewidth]{figures/bank-organization}
%  }
%
%  \caption{A DRAM bank consists of tiles and subarrays.}
%  \label{fig:bank-organization}
%\end{figure}


==> plots/subarray-service-timeline.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{plots/subarray-service-timeline-fig}
\end{center}
\caption{Service timeline of a refresh and a read request to two
different subarrays within the same bank.}
\label{fig:subarray-service-timeline}
\end{figure}


==> sec/0106-1-intro-v2.tex <==
\section{Introduction} \label{sec:intro}

Modern main memory is predominantly built using \emph{dynamic random access
memory} (DRAM) cells. A DRAM cell consists of a capacitor to store one bit of
data as electrical charge and a single transistor to access the stored data. The
capacitor leaks charge over time in a DRAM cell, causing stored data to change.
As a result, DRAM requires an operation called \emph{refresh} that periodically
reads and writes data stored in DRAM cells to maintain data integrity.

DRAM refresh is one of the performance bottlenecks for systems using DRAM as the
main memory. Because DRAM becomes unavailable to serve memory requests during
refreshes in modern DRAM devices (e.g., DDR and LPDDR
DRAM~\cite{jedec-ddr3,jedec-lpddr3}), refreshes
decrease system performance significantly (12.4\% on an 8-core system
using 8Gb DDR3 DRAM). This problem will likely become worse as DRAM density
increases, because it requires higher latency to refresh more
cells~\cite{liu-isca2012, nair-hpca2013,stuecheli-micro2010}. DRAM density is
expected to increase to 32Gb by 2020 as it doubles every two to three
years~\cite{itrs-dram}. Our evaluation shows that using 32Gb DRAM reduces system
performance by 29\% on a memory-intensive 8-core system. Therefore, it is
important to develop practical mechanisms for mitigating DRAM refresh penalties.
To help alleviate the refresh penalty, modern DRAM supports two refresh related
techniques: 1) allowing flexible refresh scheduling and 2) performing refresh in
parts of DRAM separately.

%Unfortunately, refresh is one of the performance bottlenecks for systems using
%DRAM as the main memory. Performing refresh operations decreases system
%performance because the entire DRAM rank becomes unavailable to serve memory
%requests during refresh operations in modern DRAM devices (e.g.,
%DDR~\cite{jedec-ddr3} and LPDDR~\cite{jedec-lpddr3}), increasing memory
%latency.  This problem will likely exacerbate as DRAM scales to higher density,
%requiring longer refresh operations to refresh more
%cells~\cite{stuecheli-micro2010, liu-isca2012, nair-hpca2013}.
%
%A memory controller periodically sends a refresh command, also called an
%\emph{all-bank} refresh, to a rank of DRAM devices to perform refresh
%operations on every bank within a rank simultaneously. It follows a fixed
%schedule based on a refresh interval timer for simplicity. Because a refresh
%operation prevents a memory rank from serving memory requests, performing
%refresh causes interference and delays in-flight memory requests. To help
%alleviate the refresh penalty, modern DRAM supports two refresh related
%techniques: 1) performing refresh for each bank separately and 2) allowing
%flexible refresh scheduling.


\todo{Talk about refresh scheduling: 1. 64/32ms 2. in bulk (expensive) 3.
distributed across X refs with a fixed schedule. A command refs 1/x cells. }
The first technique offers refresh scheduling flexibility by allowing refresh
commands to be issued late or early without following a static refresh
schedule~\cite{jedec-ddr3}. Taking advantage of this flexibility, one prior
work~\cite{stuecheli-micro2010} proposes \emph{elastic refresh} in attempt to
predict when the DRAM will remain idle for a sufficiently long period of time
to cover refresh latency. Then it issues all-bank refresh commands
during such periods. We find that this technique, while being effective at
improving performance, does not fully leverage the provided scheduling
flexibility and provides limited performance benefits as explained in
Section~\ref{sec:multi-core-results} and one prior work~\cite{nair-hpca2013}.

Modern DRAM is composed of multiple independent physical structures called
\emph{banks} (we will discuss banks in more detail in Section~\ref{sec:background}).
The reason DRAM becomes unavailable during a typical refresh operation is that
it refreshes every bank in parallel, preventing them from serving requests.
Thus, a typical refresh is also called an \emph{all-bank refresh}. The second
existing technique that helps to mitigate refresh penalty splits up an all-bank
refresh into multiple smaller chunks of refresh called \emph{per-bank refresh}
(only supported in LPDDR now~\cite{jedec-lpddr3, micronLPDDR2_2Gb}). In contrast
to all-bank refresh that locks up DRAM to refresh every bank, per-bank
refresh allows partial access to DRAM by refreshing only one bank at a time in a
\emph{round-robin order}. While a single bank is refreshing,
the other non-refreshing banks can serve memory accesses. But, we find that
per-bank refresh does not maximize the potential benefit from overlapping
refreshes with accesses. It can degrade system performance compared to the
conventional all-bank refresh when the system lacks bank-level parallelism to
utilize the available banks during
refresh(Section~\ref{sec:multi-core-results}).

Our goal is to mitigate the detrimental performance impact of refreshes in a way
that improves system performance over existing refresh schemes. Our key idea is
to hide refresh latency by \emph{parallelizing} refresh operations with memory
accesses to avoid delaying the latency-critical read accesses.  To this end, we
propose two complementary techniques.

The first technique, \emph{\darplong (\darp)}, is a new refresh scheduling
policy based on two key ideas: \emph{\ooolong} and \emph{\warplong}. The first
idea enables the memory controller to specify an idle bank to be refreshed as opposed
to state-of-the-art per-bank refresh policy that refreshes banks in a
round-robin order~\cite{jedec-lpddr3}. By monitoring the request queues'
occupancy, \darp avoids refreshing a bank that has pending memory requests and
instead refreshes an idle bank to maximize parallelization of refreshes and
accesses. The second idea hides refresh latency with write accesses by actively
scheduling per-bank refreshes during the time period when banks are serving
write requests. There are two major reasons why we attempt to parallelize
refresh operations with write accesses. First, modern systems typically buffer
write requests in memory controllers and drain them to the memory in a batch to
mitigate the \mbox{\emph{bus turnaround}} penalty~\cite{chatterjee-hpca2012,
stuecheli-isca2010}. Write batching allows our mechanism to proactively schedule
per-bank refresh to a bank while other banks are serving the accumulated write
requests, thus enabling more parallelization of refresh and writes to hide
refresh latency. Second, unlike read requests, write requests are not
latency-critical because a processor does not stall to wait for them to finish.
Therefore, a write request can be delayed for some period of time without
affecting performance. Taking advantage of this observation, \ib selects a bank
with a few writes to perform refresh.

Our second technique takes advantage of the fact that a DRAM bank is composed of
multiple \emph{subarrays} and each subarray has its own local \emph{sense
amplifiers}~\cite{itoh-vlsi, kim-isca2012,
moon-isscc2009,vogelsangmoon-micro2010}. We observe that only a few subarrays
are refreshed within a bank when the other subarrays and the DRAM I/O bus
remain completely idle. Based on this observation, we propose our second
technique, \emph{\intersub (\is)}. It enables a bank to be accessible during
refreshes by servicing refreshes to a few subarrays in parallel with read or write
requests to other idle subarrays, reducing the interference of refreshes on
demand requests at the cost of very modest modifications to DRAM devices.

We make the following major \textbf{contributions}: \begin{itemize}

\item We propose a new per-bank refresh scheduling policy, \darp (\darplong), to
proactively schedule refreshes to banks that are idle or that are draining
writes.

\item We propose a new DRAM refresh mechanism,
\is (\intersub), to enable a bank to serve memory requests in idle subarrays
while other subarrays are being refreshed.

%\item We perform extensive evaluations and analysis of \emph{per-bank} refresh
%mode. We show that it improves performance when there are sufficient memory
%request streams provided in a multi-core system to exploit its benefit of
%\mbox{bank-level} parallelism, but degrades performance in a single-core system
%with limited amount of outstanding memory requests.

%We evaluate our proposed mechanisms on multi-core systems with various DRAM
%densities and show that they improve system performance significantly.

\item Combining the two complementary mechanisms improves system performance of an 8-core
system by 3.3\%/7.2\%/15.2\% on average across 100 workloads and up to
7.1\%/14.5\%/27.0\% over per-bank refresh for 8/16/32Gb DRAM devices. Compared
to previously proposed elastic refresh~\cite{stuecheli-micro2010}, our mechanisms improve system
performance significantly (Section~\ref{sec:multi-core-results}).
%by 6.0\%/10.7\%/18.7\% for 8/16/32Gb DRAM devices in multi-core systems.

\end{itemize}


==> sec/0108-intro.tex <==
\section{Introduction} \label{sec:intro}

Modern main memory is predominantly built using \emph{dynamic random access
memory} (DRAM) cells. A DRAM cell consists of a capacitor to store one bit of
data as electrical charge. The capacitor leaks charge over time in a DRAM cell,
causing stored data to change. As a result, DRAM requires an operation called
\emph{refresh} that periodically restores electrical charge in DRAM cells to
maintain data integrity.

Each DRAM cell must be refreshed once every time interval specified by the DRAM
standards~\cite{jedec-ddr3,jedec-lpddr3}.
The exact refresh interval time depends on the DRAM type (e.g., DDR or LPDDR)
and the operating temperature.
Because modern DRAM devices contain
billions of cells, refreshing all of them in succession incurs high
unavailability. Instead, memory controllers send 8192 refresh commands that are
evenly distributed with a fixed schedule time between two commands throughout
the refresh interval~\cite{jedec-ddr3,jedec-lpddr3,nair-hpca2013}. As a result, each refresh
command refreshes exactly $\sfrac{1}{8192}$ of cells in DRAM. When DRAM receives
a refresh command, it starts to perform refresh operations that cause DRAM to
become unavailable to serve memory requests. The refresh latency significantly
degrades system performance~\cite{liu-isca2012, mukundan-isca2013,
nair-hpca2013,stuecheli-micro2010} by delaying in-flight memory requests (12.4\%
performance degradation on an 8-core system using 8Gb DDR3 DRAM). This problem
will likely become worse as DRAM density increases because it requires higher
latency to refresh more cells per refresh command with the same number of total
refresh commands~\cite{jedec-ddr3,jedec-lpddr3}.
DRAM density is expected to increase to 32Gb
by 2020 as it doubles every two to three years~\cite{itrs-dram}. Our evaluations
show that using 32Gb DRAM reduces system performance by 29\% on a
memory-intensive 8-core system. Therefore, it is important to develop
mechanisms to mitigate DRAM refresh penalty.

Modern DRAM is composed of multiple independent physical structures called
\emph{banks} (we will discuss banks in more detail in
Section~\ref{sec:background}). The reason DRAM becomes unavailable during a
typical refresh operation is that it refreshes every bank in parallel,
preventing them from serving requests. Thus, a typical refresh is also called an
\emph{all-bank refresh}. To help alleviate refresh latency, LPDDR
DRAM~\cite{jedec-lpddr3, micronLPDDR2_2Gb} supports a refresh mode that splits
up an all-bank refresh into multiple smaller groups of refreshes. Each of these
refreshes is called a \emph{per-bank refresh} and it is issued periodically to
only one bank at a time in a \emph{round-robin order} as opposed to the entire
DRAM. In contrast to using all-bank refresh that locks up DRAM by refreshing
every bank, using per-bank refresh allows partial access to DRAM, specifically
the non-refreshing banks, while a single bank is under refresh. Our evaluations
show that per-bank refresh improves system performance by 4.0\% over the
conventional all-bank refresh on an 8-core system. But, we find that per-bank
refresh does not maximize the potential benefit from overlapping refreshes with
accesses across banks. It can even degrade system performance compared to
all-bank refresh when the system cannot sufficiently utilize the available banks
during refresh (Section~\ref{sec:multi-core-results}).

%Our goal is to mitigate the detrimental performance impact of refreshes in a way
%that improves system performance over existing refresh schemes.

Our goal is to mitigate the detrimental performance impact of refreshes. The key
idea is to hide refresh latency by \emph{parallelizing} refresh operations with
memory accesses to avoid delaying the latency-critical read accesses. To this
end, we propose two complementary techniques.

The first technique, \emph{\darplong (\darp)}, is a new refresh scheduling
policy based on two key ideas: \emph{\ooolong} and \emph{\warplong}. The first
idea enables the memory controller to specify an idle bank to be refreshed as opposed
to state-of-the-art per-bank refresh policy that refreshes banks in a
round-robin order~\cite{jedec-lpddr3}. By monitoring the request queues'
occupancy, \darp avoids refreshing a bank that has pending memory requests and
it instead refreshes an idle bank to maximize parallelization of refreshes and
accesses. The second idea hides refresh latency with write accesses by actively
scheduling per-bank refreshes during the time period when banks are serving
write requests. There are two major reasons why we attempt to parallelize
refresh operations with write accesses. First, modern systems typically buffer
write requests in memory controllers and drain them to the memory in a batch.
%to mitigate the \mbox{\emph{bus turnaround}} penalty~\cite{chatterjee-hpca2012,
%stuecheli-isca2010}.
Write batching allows our mechanism to proactively schedule
per-bank refresh to a bank while other banks are serving the accumulated write
requests, thus enabling more parallelization of refresh and writes to hide
refresh latency. Second, unlike read requests, write requests are not
latency-critical because a processor does not stall to wait for them to finish.
Therefore, a write request can be delayed for some period of time without
affecting performance. Taking advantage of this observation, \ib selects a bank
with a few writes to perform per-bank refresh.

Our second technique takes advantage of the fact that a DRAM bank is composed of
multiple \emph{subarrays} and each subarray has its own local \emph{sense
amplifiers}~\cite{itoh-vlsi, kim-isca2012,
moon-isscc2009,vogelsangmoon-micro2010}. We observe that only a few subarrays
are refreshed within a bank when the other subarrays and the DRAM I/O bus
remain completely idle. Based on this observation, we propose our second
technique, \emph{\intersub (\is)}. It enables a bank to be accessible during
refreshes by serving refreshes to a few subarrays in parallel with read or write
requests to other idle subarrays, reducing the interference of refreshes on
demand requests at the cost of very modest modifications to DRAM devices.

We make the following major \textbf{contributions}: \begin{itemize}

\item We propose a new per-bank refresh scheduling policy, \darp (\darplong), to
proactively schedule refreshes to banks that are idle or that are draining
writes.

\item We propose a new DRAM refresh mechanism,
\is (\intersub), to enable a bank to serve memory requests in idle subarrays
while other subarrays are being refreshed.

%\item We perform extensive evaluations and analysis of \emph{per-bank} refresh
%mode. We show that it improves performance when there are sufficient memory
%request streams provided in a multi-core system to exploit its benefit of
%\mbox{bank-level} parallelism, but degrades performance in a single-core system
%with limited amount of outstanding memory requests.

%\item Combining the two complementary mechanisms improves system performance of an 8-core
%system by 3.3\%/7.2\%/15.2\% on average across 100 workloads and up to
%7.1\%/14.5\%/27.0\% over per-bank refresh for 8/16/32Gb DRAM devices. Compared
%to previously proposed elastic refresh~\cite{stuecheli-micro2010}, our mechanisms improve system
%performance significantly (Section~\ref{sec:multi-core-results}).

\item The combination of the two mechanisms (\emph{DSARP}) improves system performance of an 8-core
system by 3.3\%/7.2\%/15.2\% on average across 100 workloads and up to
7.1\%/14.5\%/27.0\% over per-bank refresh for 8/16/32Gb DRAM devices.

\end{itemize}


==> sec/7-related_dhl.tex <==
\section{Related Work}
\label{sec:related}

To our knowledge, this is the first work to comprehensively study the effect of
per-bank refresh and propose a refresh scheduling policy built on top of
per-bank refresh. We also propose a mechanism that achieves parallelization of
refresh and memory accesses within a refreshing bank. In this section, we
discuss prior works that mitigate the negative effects of DRAM refresh and
compare them to our mechanisms.

%To our knowledge, this is the first work to comprehensively study the effect
%of per-bank refresh and propose a refresh scheduling policy that is built on
%top of per-bank refresh. In addition, we propose a mechanism that achieves
%parallelization of refresh and memory accesses within a refreshing bank. In
%this section, we discuss prior works that have proposed different mechanisms
%to mitigate the negative effects of DRAM refresh. We refer a refresh as a
%conventional \mbox{all-bank} refresh unless stated otherwise.

\textbf{Refresh Scheduling.} Stuecheli et al.~\cite{stuecheli-micro2010}
propose elastic refresh that is discussed and evaluated in
Section~\ref{sec:evaluation}. In sum, elastic refresh has two shortcomings.
First, it becomes less effective when the average idle period is shorter than
\trfc as the refresh latency cannot be fully
hidden in the idle period. This occurs when
using more memory-intensive workloads with less idleness and
higher density DRAM with longer \trfc.
Second, elastic refresh incurs more refresh latency
when it incorrectly predicts a time period that has pending requests as idle.
In contrast to elastic refresh, our mechanisms parallelize refresh operations
with accesses even if there is no idle period.

%\textbf{Refresh Scheduling.} Stuecheli et al.~\cite{stuecheli-micro2010}
%propose a mechanism, elastic refresh, that we have already explained and
%compared to in Section~\ref{sec:evaluation}. In sum, elastic refresh has three
%shortcomings.  First, it becomes less effective when the average idle period
%is shorter than \trfc as the refresh latency cannot be fully hidden in the
%idle period. Second, it has less opportunity to find long idle periods to
%schedule a refresh operation for more memory-intensive workloads and for
%higher density DRAM that has longer \trfc values. Third, elastic refresh
%incurs more refresh latency when it incorrectly predicts a time period that
%has pending requests as idle. In contrast to our mechanisms, elastic refresh
%does not parallelize refresh operations with accesses and it requires idle
%periods. As a result, our mechanisms are more effective when there is no idle
%period as we parallelize refresh operations with accesses to hide refresh
%latency.

Ishii et al.~\cite{ishii-msc2012} propose a write scheduling policy that
prioritizes write draining over read requests in a rank while another rank is
refreshing even if the write queue hasn't reached the threshold. While
this technique is only applicable in multi-rank memory systems, our
mechanisms are also applicable to single-rank memory systems by enabling
parallelization of refreshes and accesses at the bank and subarray level.

%Ishii et al.~\cite{ishii-msc2012} propose a write scheduling policy that
%prioritizes write draining over read requests in a rank while another rank is
%performing refresh even if the write queue hasn't reached the threshold.
%However, it is unclear why the proposal prioritizes writes over reads when a
%rank can serve any type of requests independently of another rank. In addition,
%this technique is only applicable in a multi-rank memory subsystem. Our
%mechanisms differ from theirs as we enable parallelization
%of refresh and memory accesses at the bank and subarray level.

Mukundan et al.~\cite{mukundan-isca2013} propose scheduling techniques in
addition to adaptive refresh discussed in Section~\ref{sec:ddr4} to address the
problem of command queue seizure, whereby a command queue gets filled up with
commands to a refreshing rank, blocking commands to another non-refreshing rank.
In our work, we use a different memory controller design that does not have
command queues as similar to prior work~\cite{herrero-tc2013}. The key
distinction is that our controller generates a command for a scheduled request
right before it is sent to DRAM instead of pre-generating the commands and
queueing them up. Thus, our design does not suffer from command queue seizure.

%In addition to adaptive refresh discussed in Section~\ref{sec:ddr4}, Mukundan et
%al.~\cite{mukundan-isca2013} propose other scheduling techniques to address the
%problem of command queue seizure, whereby a command queue gets filled up with
%commands to a refreshing rank, blocking commands to another non-refreshing rank.
%In our work, we use a different memory controller design that does not have
%command queues. The key distinction is that our controller generates a command
%for a scheduled request right before it is sent to DRAM instead of
%pre-generating the commands and queueing them up. Thus, our design ensures that
%command queue seizure does not happen. A similar design has been used in prior
%work~\cite{herrero-tc2013}.

\textbf{Subarray-Level Parallelism.} Kim et al. propose a technique called
“subarray-level parallelism” (SALP)~\cite{kim-isca2012} to reduce bank
serialization latency by enabling multiple accesses to different subarrays
within a bank to proceed in parallel. In contrast to SALP, our mechanism (\is)
parallelizes refreshes and accesses to different subarrays within the same bank.
As described in Section~\ref{sec:sarp_implementation}, we reduce the sharing of the
peripheral circuits for refreshes and accesses. Such an implementation regarding
refresh is not discussed and explored in SALP. Therefore, \is enables
independent subarray operations in a different way from SALP.

%\textbf{Subarray-Level Parallelism.} Kim et al. propose a technique called
%“subarray-level parallelism” (SALP)~\cite{kim-isca2012} to improve DRAM
%performance. SALP reduces bank serialization latency by enabling multiple
%accesses to different subarrays within a bank to proceed in parallel. The key
%difference between \is (our proposal) and SALP is that unlike \is, SALP cannot
%parallelize a refresh operation in one subarray with an access to another
%subarray in the same bank. In SALP, a single row counter provides the refresh
%row address that passes through the row-address MUX shared with the row address
%provided by the memory controller as shown in \figref{detail-bank-organization}.
%Because a single refresh command initiates a \emph{sequence} of rows to be
%refreshed internally, the memory controller is oblivious to when the refresh
%logic is sending the refresh row address through the bus to the row-address MUX.
%As a result, an externally issued command can collide with a refresh row address
%within a bank, resulting in unknown outcome for the external command from the
%memory controller. To solve this problem, we reduce the sharing of the
%peripheral circuits for the refresh row address and the externally issued row
%address within a bank. Specifically, we separate the row counter into two
%separate counters and route these counters with global wires across the bank to
%provide refresh selection. Such a modification along with the appropriate bank
%control logic enables \is to parallelize refreshes with accesses, which cannot
%be achieved with the current implementation of SALP.

\textbf{Refresh Pausing.} Nair et al.~\cite{nair-hpca2013} propose refresh
pausing that pauses a refresh to serve memory requests. To make pausing a
refresh possible, the authors assume that DRAM refreshes multiple rows
\emph{sequentially}. Thus, there is a short recovery time, called a "refresh
pausing point" (RPP), after refreshing each row so that the memory controller
can signal the DRAM to stop refreshing subsequent rows. However, DRAM
manufacturers currently design their chips to refresh multiple rows in
\emph{parallel} (staggered/pipelined as explained in ~\cite{mukundan-isca2013}).
Therefore, the current implementation of refresh pausing requires modification
to become effective in modern DRAM due to lack of RPPs.

%The authors show that
%the latency to refresh eight rows ($8 \times \trc$) individually by issuing
%explicit activation commands from a memory controller is \emph{less} than the
%refresh latency (\trfc) resulting from a refresh command.
%However, DRAM manufacturers currently design their chips to refresh multiple
%rows in \emph{parallel} (staggered/pipelined as explained in
%~\cite{mukundan-isca2013}). The current 8Gb DDR3 DRAM data
%sheets~\cite{jedec-ddr3,micronDDR3_8Gb} actually show that 8 $\times$ \trc $>$
%\trfc with \trc ranging from 45ns to 52.5ns (as opposed to 39ns used
%in~\cite{nair-hpca2013}) with \trfc remaining at 350ns.
%ddr4: 44.5ns - 50ns
%ddr3-1066: 50.625 for the exact same params as in the micron datasheet

%\textbf{Refresh Pausing.}
%Nair et al.~\cite{nair-hpca2013} propose refresh pausing in attempt to pause a
%refresh to serve memory requests. To make pausing a refresh possible, the
%authors assume that there is a short recovery time, called a "refresh pausing
%point" (RPP), after refreshing each row so that the memory controller can signal
%the DRAM to stop refreshing subsequent rows. The reason RPPs exist is that they
%assume rows are \emph{sequentially} refreshed during refresh and the latency
%to refresh eight rows sequentially ($8 \times \trc$) is \emph{less} than the
%refresh latency (\trfc). However, DRAM manufacturers currently design their
%chips so that multiple rows are refreshed in \emph{parallel}
%(staggered/pipelined as explained in ~\cite{mukundan-isca2013}). Using the same
%8Gb DDR3 DRAM data sheets~\cite{jedec-ddr3,micronDDR3_8Gb} actually shows that
%8 $\times$ \trc $>$ \trfc with \trc ranging from 45ns to 52.5ns (as opposed
%to 39ns used in their paper) with \trfc remaining at 350ns. Therefore, to make
%refresh pausing viable, one would need to justify the existence of Refresh
%Pausing Points.

\textbf{eDRAM Concurrent Refresh.} Kirihata et al.~\cite{kirihata-jssc2005}
propose a mechanism to enable a bank to refresh independently while another
bank is being accessed in embedded DRAM (eDRAM). Our work differs
from~\cite{kirihata-jssc2005} in two important ways. First, unlike SARP, their
proposal parallelizes refreshes only across banks and not within banks.
Second, there are significant differences between DRAM and eDRAM architectures,
which make it non-trivial to apply their technique directly to DRAM
architectures. In particular, eDRAMs have no standardized timing/power
integrity constraints and access protocol, making it simpler for each bank to
independently manage its refresh schedule. In contrast, refreshes in DRAM need
to be managed by the memory controller to ensure that parallelizing refreshes
with accesses does not violate other constraints.

%\textbf{eDRAM Concurrent Refresh.} Kirihata et al.~\cite{kirihata-jssc2005}
%propose a mechanism to enable a bank to refresh independently while another bank
%is being accessed in embedded DRAM (eDRAM). Our work differs
%from~\cite{kirihata-jssc2005} in two important ways. First, unlike SARP, their
%proposal parallelizes refreshes only across banks and not within banks. In this
%regard, their work shares more similarities with per-bank refresh in LPDDR
%DRAMs. Second, there are significant differences between DRAM and eDRAM
%architectures, which make it non-trivial to apply their technique directly to
%DRAM architectures. In particular, eDRAMs have no standardized timing/power
%integrity constraints and access protocol, making it simpler for each bank to
%independently manage its refresh schedule. In contrast, refreshes in DRAM need
%to be managed by the memory controller to ensure that parallelizing refreshes
%with accesses does not violate other constraints.

\textbf{Retention-Aware Refresh.} Prior works (e.g.,~\cite{liu-isca2012,
venkatesan-hpca2006}) have proposed mechanisms to take advantage of the fact
that DRAM cells leak charge at different rates due to various factors, such as
process variation, leading to different retention time for each cell. However,
these prior works have the same disadvantage of assuming that the retention
time of DRAM cells can be \emph{accurately} profiled and their mechanisms all
depend on having this profile in order to guarantee that DRAM refresh is
handled in a timely manner. Ensuring profile accuracy has the difficulties of
facing physical phenomena of Variable Retention Time (VRT) and Data Pattern
Dependence (DPD)~\cite{liu-isca2013} that can cause the retention time of a
cell to fluctuate over time. Therefore, these mechanisms need to overcome the
profiling challenges to be viable.


==> sec/algos/interbank-algo.tex.0527 <==
\begin{algorithm}
\caption{\small Parallelizing Refreshes with Write Requests}
\label{algo:interbank-algo}
\footnotesize{
\textbf{\underline{Definition:}}
\begin{algorithmic}
\STATE \begin{itemize}
    \item \textit{N}: number of banks per rank
    \item \textit{write\_queue[N]}: an array of queues storing write requests
    \item \textit{refresh\_queue[N]}: an array of queues storing refresh requests
    \item \textit{ref\_credit[N]}: an array of credits keeping track of the number of
    postponed and pulled-in refreshes
    \item \textit{next\_ref\_bank}: the bank to be refreshed next after \trefi refreshes
    \item \textit{max\_postpone}: maximum number of allowed postponed refreshes
    \item \textit{max\_pull}: maximum number of allowed pulled-in refreshes
    \item \textit{refreshBank(b)}: refresh the specified bank
    \end{itemize}
\end{algorithmic}

\textbf{\underline{Every tREFI:}}
\begin{algorithmic}
\IF{\textit{ref\_credit[\textit{next\_ref\_bank}]} > -\textit{max\_postpone}}
    \STATE \textit{ref\_credit[\textit{next\_ref\_bank}]} -= 1
    \COMMENT {Postpone refresh}
\ELSE
    \STATE \textit{refreshBank(\textit{next\_ref\_bank})}
\ENDIF
\end{algorithmic}

\textbf{\underline{During Writeback Mode:}}
\begin{algorithmic}
\IF {no write request is scheduled}
\FOR{\textbf{each} $b$ in N}
    \IF {$refresh\_queue[b].isEmpty()$ AND $b.isIdle()$ AND $ref\_credit[b] <
    max\_pull$ AND $\frac{\trc \times
    write\_requests\_left} {writeback\_BLP} > tRFC$}
        \STATE \textit{refreshBank($b$)}
        \COMMENT {Issue either a postponed or pulled-in refresh}
        \STATE \textit{ref\_credit[$b$]} += 1
        \STATE break
    \ENDIF
\ENDFOR
\ENDIF
\end{algorithmic}
}
\end{algorithm}


==> sec/algos/ooo-algo.tex <==
\begin{algorithm}
\caption{\small \ooolongCap}
\label{algo:ooo-algo}
\footnotesize{
\textbf{\underline{Definition:}}
\begin{algorithmic}
\STATE \begin{itemize}
    \item \textit{ref\_credit[number of banks]}: an array of credits keeping track of the number of
    postponed and pulled-in refreshes
    \item \textit{max\_postpone}: maximum number of allowed postponed refreshes
    \item \textit{max\_pull}: maximum number of allowed pulled-in refreshes
    \item \textit{refresh\_candidate}: a list of bank IDs with no
    pending read requests
    \item \textit{ref\_bank}: the bank to be refreshed in the sequential
    round-robin order
    \end{itemize}
\end{algorithmic}

\textbf{\underline{Every tREFI:}}
\begin{algorithmic}
\IF{\textit{ref\_credit[\textit{ref\_bank}]} > -\textit{max\_postpone}}
    \STATE \textit{ref\_credit[\textit{ref\_bank}]} -= 1
    \COMMENT {\textbf{Postpone refresh}}
\ELSE
    \STATE \textit{refreshBank(\textit{ref\_bank})}
    \COMMENT {\textbf{A forced refresh}}
\ENDIF
\end{algorithmic}

\textbf{\underline{Every Cycle:}}
\begin{algorithmic}
\IF{no demand request issued}
    \FOR{\textbf{each} \textit{bank} in \textit{refresh\_candidate}}
        \IF{-\textit{max\_postpone} < \textit{ref\_credit[\textit{bank}]} <
        \textit{max\_pull}}
            \STATE \textit{refreshBank(\textit{bank})}
            \COMMENT {\textbf{Either a postponed or pulled-in refresh}}
            \STATE break
        \ENDIF
    \ENDFOR
\ENDIF
\end{algorithmic}
}
\end{algorithm}

